Modeling Knowledge Acquisition from Multiple Learning Resource Types

Students acquire knowledge as they interact with a variety of learning materials, such as video lectures, problems, and discussions. Modeling student knowledge at each point during their learning period and understanding the contribution of each learning material to student knowledge are essential for detecting students' knowledge gaps and recommending learning materials to them. Current student knowledge modeling techniques mostly rely on one type of learning material, mainly problems, to model student knowledge growth. These approaches ignore the fact that students also learn from other types of material. In this paper, we propose a student knowledge model that can capture knowledge growth as a result of learning from a diverse set of learning resource types while unveiling the association between the learning materials of different types. Our multi-view knowledge model (MVKM) incorporates a flexible knowledge increase objective on top of a multi-view tensor factorization to capture occasional forgetting while representing student knowledge and learning material concepts in a lower-dimensional latent space. We evaluate our model in different experiments toshow that it can accurately predict students' future performance, differentiate between knowledge gain in different student groups and concepts, and unveil hidden similarities across learning materials of different types.

==> reviews/reviews.tex <==
1: (weak accept)
Overall, this paper covers a critical topic and stresses the importance of modeling student knowledge from multiple learning materials. The problem formulation and assumptions are well thought of and explained.

I would be interested in learning more on why the particular MOOCs course data are considered the most appropriate real-world choice to study the research question.

It is very interesting to learn of the MVKM model to discover materials’ latent concepts. I would want to see more elaboration on this. What is the motivation to do so and what are some of the implications of doing so?

There is also a lack of discussion on possible influence from course features in addition to videos, discussions, and quizzes.


1: (weak accept)
Authors propose a multi-view student knowledge model (MVKM) that can capture learning from multiple learning material types. It nicely establishes the assumptions on which their student knowledge model is built and subsequently describes how those assumptions are incorporated in the model. The major contributions are as follows 1) A nice addition of Multi-view student knowledge model in education data mining methods based on a well-thought tensor factorization method 2) Authors have put substantial efforts on interpretability of their model which is appreciable 3) Empirical results on synthetic and real world datasets are encouraging.
However, there are several places where the paper can be improved.

The problem formulation context would be easy to digest with some illustrative examples instead of being introduced in abstract format. For example, it does immediately become clear what set of $P^[r]$ learning materials authors are referring to initially. I see abuse of notations at several places. For example, using notation without describing them first such as in Section 3.2 (see $\hat{x}_{s, a,p}, s_{s}, T_a, q_p$).

What is "t" in Equation 2? There are other better ways to enforce temporal smoothness in student performance (something along kernel smoothing) and thus Equation (2) formulation requires more effort and motivation but seems reasonable.

It is not clear whether enforcing the sum-one constraint on each student's membership in the student latent features is required?

It is also not clear whether an assumption on the feedback score function or metric is needed because authors expect student scores in attempt a+1 to be more than their scores in attempt a. This requirement put constraint on the score function that can be adopted for a learning material to resonate with the above expectation.

Importantly, computational complexity of their tensor factorization approach is missing. The scalability of their proposed method is doubtful and needs to be discussed.

Evaluation methodology seems convincing and empirical results are promising and in depth model analysis in section 4.4 and section 4.5 portrays the value of their multi-view learning approach.


2: (accept)
1) summary
This paper presents a novel model (called the multi-view knowledge model) for integrating student interaction with multiple types of learning materials in a course. The model is compared with several standard methods in EDM for prediction of learning from the first half of a course to the second half. The paper has interesting results when tests on both simulated and actual course data and the authors do a nice job of exploring the resulting models and whether they align with intuition about student performance and learning.

2) Recommendation: accept
This paper presents a novel method for course participation analysis and prediction of performance and presents good ways to do comparisons across models.

3) reasons for recommendation

The proposed models are clearly interesting, and the analyses show that the new models can find differences between resource types. It will be exciting to see these methods applied to other data sets.

4) suggestions for improvement

I would have liked a slightly longer discussion or a little more elaboration on some of the most interesting points. I liked the clustering in figures 6 and 7. Good use of colors and boxes. It was also nice to see some examples of student learning predictions and the intuitive analysis of each.

Some specific corrections are suggested below.

Specific comments:
P2 "while annotated students
may help students to learn, weaker students may study more
annotated examples [22]."
->
"while annotated examples
may help students to learn, weaker students may study more
annotated examples [22]."

P3
"knowledge increase happens
as a result of student interaction with non-graded material."
->
"knowledge increases that happen
as a result of student interaction with non-graded material."

P3
"is a matrix capture the relationship"
->
"is a matrix capturing the relationship"

P6
"does not have constraint that student knowledge is inscreaing."
->
"does not have constraint that student knowledge is increasing."




The reviewers felt that this paper on multi-view knowledge models was interesting and provided a novel method for analyzing student participation data in courses with multiple learning material types.

The paper could be improved with some more elaboration on the specifics of the choices for the course and materials used. Specifically, the authors should elaborate more on the limitations and generalizability of the methods and results -If I recall correctly, the models only really looked at one type of resource versus all others. But it was not entirely clear.


%------------------------------------------------

% 1. problem formulation, explain in more clear way
% 2. notation recheck, eg. equation 1, eq 2
% 3. why we have this score increasing assumption, explain in more clear way
% 4. explain the reason why use eq 2 as constraint more clearly
% 5. we don't sum S as 1, delete this in eq 3
% 6. computational complexity and scalability need to be discussed
% 7. correct the typos/grammar in reviews 3
